MLAAD: The Multi-Language Audio Anti-Spoofing Dataset

This paper presents the Multi-Language Audio Anti-Spoofing Dataset (MLAAD), version 11: a dataset of synthetic audio to train and evaluate audio deepfake detection models. It features 205 Text-to-Speech (TTS) models, comprising a total of 1153.6 hours of synthetic voice in 54 different languages. To evaluate this dataset, we train three state-of-the-art deepfake detection models with MLAAD and observe that it demonstrates superior performance to comparable datasets like InTheWild and FakeOrReal when used as a training resource. Moreover, compared to the renowned ASVspoof 2019 dataset, MLAAD proves to be a complementary resource. In tests across eight datasets, MLAAD and ASVspoof 2019 alternately outperformed each other, each excelling on four datasets. By publishing the dataset and making a trained model accessible via an interactive webserver, we aim to democratize anti-spoofing technology, making it accessible beyond the realm of specialists, and contributing to global efforts against audio spoofing and deepfakes.

==> data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 2.7 \\
Capacitron & 1.5 \\
FastPitch & 2.1 \\
GlowTTS & 8.1 \\
Griffin Lim & 16.6 \\
Jenny & 1.7 \\
Mars5 & 1.8 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
NeuralHMM & 2.1 \\
Overflow & 2.2 \\
Parler TTS & 1.7 \\
SpeechT5 & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 2.0 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 3.9 \\
Tortoise & 2.1 \\
VITS & 39.0 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 20.5 \\
XTTS v2 & 19.7 \\
\bottomrule
\end{tabular}


==> hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 12.2 \\
Common Voice & 17.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 19.3 \\
LibriTTS & 2.0 \\
M-AILABS & 6.2 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 65.6 \\
Sam & 2.5 \\
Thorsten & 1.8 \\
WhisperSpeech dataset & 3.9 \\
none & 16.6 \\
unknown & 9.9 \\
\bottomrule
\end{tabular}


==> hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 3.3 \\
Bulgarian & 2.0 \\
Czech & 2.0 \\
Danish & 1.8 \\
Dutch & 9.6 \\
English & 48.9 \\
Estonian & 1.6 \\
Finnish & 5.1 \\
French & 12.1 \\
German & 12.2 \\
Greek & 2.2 \\
Hindi & 2.4 \\
Hungarian & 6.4 \\
Irish & 2.1 \\
Italian & 12.5 \\
Maltese & 2.0 \\
Polish & 10.5 \\
Romanian & 4.5 \\
Russian & 9.6 \\
Slovak & 2.2 \\
Spanish & 7.5 \\
Swahili & 3.4 \\
Ukrainian & 9.6 \\
\bottomrule
\end{tabular}


==> hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Mars5 & 1.8 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
WhisperSpeech & 3.9 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
microsoft/speecht5_tts & 2.0 \\
parler_tts & 1.7 \\
suno/bark & 2.7 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 20.5 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 19.7 \\
tts_models/nl/css10/vits & 2.1 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
\bottomrule
\end{tabular}


==> img/data/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
speaker_similarity \\
reference_speaker \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 284.3 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
openai & 13.7 \\
unknown & 718.2 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Audio8-TTS-Preview-0.1b & 1.8 \\
Audio8-TTS-Preview-0.6b & 1.8 \\
Ava-82M & 2.1 \\
Azzurra-Voice & 1.5 \\
CaroTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 \\
ChatTTS & 3.7 \\
Chatterbox & 1.8 \\
Chatterbox Multilingual & 10.8 \\
Chatterbox-Turbo & 1.8 \\
DeepGram & 3.8 \\
Dramabox & 3.5 \\
Echo-TTS & 2.0 \\
Edge-TTS & 39.9 \\
ElevenLabs-Turbo-v2.5 & 2.0 \\
ElevenLabs-v2-Multilingual & 4.1 \\
ElevenLabs-v3 & 4.0 \\
FireRedTTS-2.0 & 5.5 \\
Fish-S2-Pro & 19.8 \\
FishTTS & 7.4 \\
FreyaTTS & 1.6 \\
GLM-TTS & 2.1 \\
GPA-v1.0 & 1.7 \\
GPA-v1.5 & 1.8 \\
GPT-SoVITS & 2.1 \\
Gemini-3.1-Flash-TTS & 2.5 \\
Higgs-Audio-V2 & 8.8 \\
Higgs-Audio-V3 & 15.5 \\
Hume TADA-3B-ML & 14.0 \\
Index-TTS-1.5 & 4.0 \\
Index-TTS-2.0 & 3.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Inflect-Micro-v2 & 1.8 \\
Inflect-Nano-v1 & 1.5 \\
Inflect-Nano-v2 & 1.8 \\
Inworld-TTS-2 & 3.9 \\
Kani-TTS-370M & 3.8 \\
Kartoffelbox & 1.9 \\
Kitten-TTS-Nano-0.1 & 2.0 \\
Kitten-TTS-Nano-0.2 & 2.1 \\
KugelAudio & 15.6 \\
Kyutai-TTS & 4.5 \\
LEMAS-TTS & 18.5 \\
LFM2.5-Audio & 1.8 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
LongCat-AudioDiT & 3.3 \\
LuxTTS & 1.8 \\
MOSS-TTS-1.7B & 20.8 \\
MOSS-TTS-8B & 18.1 \\
MOSS-TTS-Nano-100M & 2.1 \\
Mars5 & 1.8 \\
Marvis-TTS & 1.7 \\
MatchaTTS & 1.7 \\
Maya1 TTS & 2.1 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice 1.5B & 4.1 \\
Microsoft VibeVoice Large & 4.2 \\
MingTTS & 3.9 \\
MiniCPM-o-2.6 & 4.4 \\
MiniMax-Speech-2.8-Turbo & 2.0 \\
MiraTTS & 2.0 \\
MisoTTS & 2.3 \\
NVidia Magpie-TTS Multilingual & 4.5 \\
Nari Dia-1.6B & 1.9 \\
Nari Dia2 & 2.1 \\
NeuTTS-Air & 2.0 \\
NeuTTS-Nano & 2.0 \\
OmniVoice & 53.6 \\
OpenAI TTS-1 HD & 13.7 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
OuteTTS & 15.1 \\
Parler-mini-multilingual & 10.0 \\
PocketTTS & 1.9 \\
PrimeTTS & 2.1 \\
Qwen2.5-Omni & 2.3 \\
Qwen3-TTS-12Hz-0.6B-Base & 17.3 \\
Qwen3-TTS-12Hz-1.7B-Base & 17.0 \\
Qwen3-TTS-CustomVoice & 2.3 \\
RVC & 17.6 \\
Raon-OpenTTS & 1.8 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Rime-Coda & 7.3 \\
Ringg Squirrel TTS v1.0 & 3.9 \\
Smallest-Lightning-v3.1 & 3.5 \\
Soprano11 & 1.6 \\
SopranoTTS & 1.7 \\
Sopro & 2.0 \\
SoulX-Podcast & 1.9 \\
Spark-TTS-0.5B & 2.1 \\
Step-Audio-EditX & 3.8 \\
Supertonic & 1.9 \\
SvaraTTS v1 & 5.2 \\
TADA-1B & 1.9 \\
TADA-3B-ML & 1.6 \\
Tsukasa_Speech & 4.1 \\
VITS2-Claude & 1.7 \\
Veena & 3.5 \\
VibeVoice-Realtime-0.5B & 2.0 \\
VieNeu-TTS & 2.3 \\
VoXtream2 & 1.9 \\
VoiceCore & 2.9 \\
VoxCPM-0.5B & 3.6 \\
VoxCPM-1.5 & 4.1 \\
VoxCPM2 & 32.0 \\
Voxtral & 19.1 \\
Voxtream & 2.2 \\
WavTTS & 1.7 \\
WhisperSpeech & 3.9 \\
YarnGPT & 5.2 \\
ZONOS2 & 8.8 \\
ZipVoice & 3.4 \\
dots.tts-base & 15.2 \\
dots.tts-mf & 15.1 \\
dots.tts-soar & 15.2 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
minimax/speech-02-turbo & 6.7 \\
minimax/speech-2.6-hd & 2.1 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sarashina2.2-tts & 2.2 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
supertonic-3 & 15.9 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v1/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
    training\_data & duration \\
\midrule
    Blizzard 2013 &      1.5 \\
           CSS 10 &      5.9 \\
     Common Voice &      7.8 \\
              EK1 &      1.6 \\
            Jenny &      0.7 \\
         LJSpeech &      7.7 \\
              Mai &      3.5 \\
       Mai\_female &      1.6 \\
         Mai\_male &      2.0 \\
Multiple Datasets &     23.1 \\
              Sam &      1.1 \\
         Thorsten &      1.9 \\
             none &      1.0 \\
          unknown &      1.2 \\
\bottomrule
\end{tabular}


==> img/data_v1/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
 language & duration \\
\midrule
   Arabic &      2.7 \\
Bulgarian &      0.8 \\
    Czech &      3.0 \\
   Danish &      0.7 \\
    Dutch &      3.7 \\
  English &     18.1 \\
 Estonian &      0.7 \\
  Finnish &      1.1 \\
   French &      3.7 \\
   German &      5.8 \\
    Greek &      1.0 \\
    Hindi &      1.1 \\
Hungarian &      2.0 \\
    Irish &      0.8 \\
  Italian &      6.1 \\
  Maltese &      0.8 \\
 Romanian &      0.8 \\
  Russian &      2.6 \\
   Slovak &      0.8 \\
  Spanish &      4.3 \\
  Swedish &      0.7 \\
Ukrainian &      1.8 \\
\bottomrule
\end{tabular}


==> img/data_v1/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
            model & duration \\
\midrule
             Bark &      1.2 \\
Capacitron, C=150 &      0.8 \\
 Capacitron, C=50 &      0.7 \\
        FastPitch &      0.8 \\
          GlowTTS &      3.6 \\
      Griffin Lim &      1.0 \\
            Jenny &      0.7 \\
        NeuralHMM &      0.8 \\
         Overflow &      0.8 \\
    Speedy Speech &      0.1 \\
     Tacotron DDC &      1.1 \\
        Tacotron2 &      1.6 \\
    Tacotron2 DCA &      1.9 \\
     Tacotron2 DH &      0.8 \\
    Tacotron2-DDC &      2.7 \\
         Tortoise &      0.9 \\
             VITS &     17.0 \\
        VITS Neon &      2.0 \\
        XTTS v1.1 &     11.6 \\
          XTTS v2 &     12.1 \\
          YourTTS &      0.8 \\
\bottomrule
\end{tabular}


==> img/data_v10/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
speaker_similarity \\
reference_speaker \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v10/hours_per_architecture.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l r | l r | l r@{}}
\toprule
\textbf{Architecture} & \textbf{Hours} & \textbf{Architecture} & \textbf{Hours} & \textbf{Architecture} & \textbf{Hours} \\
\midrule
Azzurra-Voice & 1.5 & Mars5 & 1.8 & Sesame CSM 1B & 2.2 \\
Bark & 123.3 & MatchaTTS & 1.7 & Sesame CSM-1B & 1.7 \\
Capacitron & 1.5 & Maya1 TTS & 2.1 & Soprano11 & 1.6 \\
CaroTTS & 1.7 & MegaTTS3 & 4.1 & SopranoTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 & MeloTTS & 1.8 & SoulX-Podcast & 1.9 \\
Chatterbox & 16.3 & Metavoice-1B & 1.9 & Spark TTS & 2.1 \\
ChatTTS & 3.7 & Microsoft VibeVoice & 8.3 & SpeechT5 & 2.0 \\
DeepGram & 3.8 & Ming-omni-tts & 3.9 & Speedy Speech & 2.0 \\
Dual-AR & 19.8 & MiniCPM-o-2.6 & 4.4 & Step-Audio-EditX & 3.8 \\
E2 TTS & 1.8 & MiniMax-Speech & 2.0 & StyleTTS 2 & 4.1 \\
Edge-TTS & 39.9 & minimax/speech-02 & 8.8 & Supertonic & 1.9 \\
ElevenLabs & 10.1 & MiraTTS & 2.0 & SvaraTTS v1 & 5.2 \\
F5 TTS & 1.7 & MOSS-TTS & 38.9 & Tacotron & 2.5 \\
F5-TTS & 18.5 & Nari Dia-1.6B & 1.9 & Tacotron 2 & 20.6 \\
FastPitch & 2.1 & Nari Dia2 & 2.1 & TADA & 17.5 \\
FireRedTTS & 5.5 & NeuralHMM & 2.1 & Tortoise & 2.1 \\
FishTTS & 7.4 & NeuTTS & 2.0 & Veena & 3.5 \\
Gemini & 2.5 & NeuTTS-Air & 2.0 & VieNeu-TTS & 2.3 \\
GLM-TTS & 2.1 & NVidia Magpie-TTS & 4.5 & VITS & 54.4 \\
GlowTTS & 12.6 & OmniVoice & 53.6 & VITS Neon & 4.3 \\
Griffin Lim & 16.6 & OpenAI TTS-1 HD & 13.7 & VITS-MMS & 23.3 \\
Higgs-Audio-V2 & 8.8 & Openaudio-S1-Mini & 4.8 & VITS2 & 1.7 \\
Index-TTS & 7.6 & OpenVoiceV2 & 4.3 & VixTTS & 3.6 \\
IndicF5 & 16.6 & Optispeech & 1.5 & VoiceCore & 2.9 \\
Indri-TTS-0.1 & 3.7 & Orpheus TTS v0.1 & 2.0 & VoxCPM & 35.6 \\
Jenny & 1.7 & OuteTTS & 15.1 & VoxCPM-1.5 & 4.1 \\
Kani-TTS & 3.8 & Overflow & 2.2 & Voxtral & 19.1 \\
Kitten-TTS & 4.1 & Parler TTS & 4.9 & VoXtream & 1.9 \\
Kokoro & 10.4 & PocketTTS & 1.9 & Voxtream & 2.2 \\
KugelAudio & 15.6 & Qwen2.5-Omni & 2.3 & WhisperSpeech & 3.9 \\
Kyutai-TTS & 4.5 & Qwen3-Omni & 34.3 & XTTS v1.1 & 36.9 \\
LFM2.5-Audio & 1.8 & Raon-OpenTTS & 1.8 & XTTS v2 & 38.9 \\
Llasa & 30.9 & Resemble.ai (April 12th, 2025) & 8.8 & YarnGPT & 5.2 \\
LongCat-AudioDiT & 3.3 & Ringg Squirrel TTS & 3.9 & ZipVoice & 3.4 \\
LuxTTS & 1.8 & RVC & 17.6 & ZonosTTS v0.1 & 3.7 \\
\bottomrule
\end{tabular*}


==> img/data_v10/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 284.3 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
openai & 13.7 \\
unknown & 567.5 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v10/hours_per_language.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l r | l r | l r@{}}
\toprule
\textbf{Language} & \textbf{Hours} & \textbf{Language} & \textbf{Hours} & \textbf{Language} & \textbf{Hours} \\
\midrule
Amharic & 3.6 & Hungarian & 12.5 & Polish & 32.3 \\
Arabic & 19.4 & Igbo & 1.8 & Portuguese & 39.2 \\
Bangla & 14.1 & Indonesian & 4.5 & Romanian & 12.8 \\
Bulgarian & 6.1 & Irish & 6.4 & Russian & 39.9 \\
Chinese & 54.6 & Italian & 45.9 & Sinhala & 2.1 \\
Croatian & 1.8 & Japanese & 29.9 & Slovak & 6.3 \\
Czech & 13.0 & Javanese & 2.4 & Slovenian & 1.8 \\
Danish & 7.7 & Kannada & 9.4 & Spanish & 50.9 \\
Dutch & 20.8 & Korean & 30.2 & Swahili & 3.4 \\
English & 232.3 & Latvian & 2.3 & Swedish & 7.4 \\
Estonian & 5.7 & Lithuanian & 2.3 & Tamil & 5.0 \\
Finnish & 13.2 & Luxembourgish & 1.7 & Thai & 7.8 \\
French & 66.6 & Malay & 2.5 & Turkish & 14.0 \\
German & 69.9 & Malayalam & 1.8 & Turkmen & 3.9 \\
Greek & 8.8 & Maltese & 8.1 & Ukrainian & 25.1 \\
Hausa & 1.5 & Marathi & 3.0 & Urdu & 2.1 \\
Hebrew & 2.0 & Norwegian & 2.0 & Vietnamese & 10.1 \\
Hindi & 22.5 & Persian & 6.7 & Yoruba & 1.8 \\
\bottomrule
\end{tabular*}


==> img/data_v10/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Azzurra-Voice & 1.5 \\
CaroTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 \\
ChatTTS & 3.7 \\
Chatterbox & 1.8 \\
Chatterbox Multilingual & 10.8 \\
Chatterbox-Turbo & 1.8 \\
DeepGram & 3.8 \\
Edge-TTS & 39.9 \\
ElevenLabs-Turbo-v2.5 & 2.0 \\
ElevenLabs-v2-Multilingual & 4.1 \\
ElevenLabs-v3 & 4.0 \\
FireRedTTS-2.0 & 5.5 \\
Fish-S2-Pro & 19.8 \\
FishTTS & 7.4 \\
GLM-TTS & 2.1 \\
Gemini-3.1-Flash-TTS & 2.5 \\
Higgs-Audio-V2 & 8.8 \\
Hume TADA-3B-ML & 14.0 \\
Index-TTS-1.5 & 4.0 \\
Index-TTS-2.0 & 3.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Kani-TTS-370M & 3.8 \\
Kartoffelbox & 1.9 \\
Kitten-TTS-Nano-0.1 & 2.0 \\
Kitten-TTS-Nano-0.2 & 2.1 \\
KugelAudio & 15.6 \\
Kyutai-TTS & 4.5 \\
LEMAS-TTS & 18.5 \\
LFM2.5-Audio & 1.8 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
LongCat-AudioDiT & 3.3 \\
LuxTTS & 1.8 \\
MOSS-TTS-1.7B & 20.8 \\
MOSS-TTS-8B & 18.1 \\
Mars5 & 1.8 \\
Marvis-TTS & 1.7 \\
MatchaTTS & 1.7 \\
Maya1 TTS & 2.1 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice 1.5B & 4.1 \\
Microsoft VibeVoice Large & 4.2 \\
MingTTS & 3.9 \\
MiniCPM-o-2.6 & 4.4 \\
MiniMax-Speech-2.8-Turbo & 2.0 \\
MiraTTS & 2.0 \\
NVidia Magpie-TTS Multilingual & 4.5 \\
Nari Dia-1.6B & 1.9 \\
Nari Dia2 & 2.1 \\
NeuTTS-Air & 2.0 \\
NeuTTS-Nano & 2.0 \\
OmniVoice & 53.6 \\
OpenAI TTS-1 HD & 13.7 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
OuteTTS & 15.1 \\
PocketTTS & 1.9 \\
Qwen2.5-Omni & 2.3 \\
Qwen3-TTS-12Hz-0.6B-Base & 17.3 \\
Qwen3-TTS-12Hz-1.7B-Base & 17.0 \\
RVC & 17.6 \\
Raon-OpenTTS & 1.8 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Ringg Squirrel TTS v1.0 & 3.9 \\
Soprano11 & 1.6 \\
SopranoTTS & 1.7 \\
SoulX-Podcast & 1.9 \\
Spark-TTS-0.5B & 2.1 \\
Step-Audio-EditX & 3.8 \\
Supertonic & 1.9 \\
SvaraTTS v1 & 5.2 \\
TADA-1B & 1.9 \\
TADA-3B-ML & 1.6 \\
Tsukasa_Speech & 4.1 \\
VITS2-Claude & 1.7 \\
Veena & 3.5 \\
VieNeu-TTS & 2.3 \\
VoXtream2 & 1.9 \\
VoiceCore & 2.9 \\
VoxCPM-0.5B & 3.6 \\
VoxCPM-1.5 & 4.1 \\
VoxCPM2 & 32.0 \\
Voxtral & 19.1 \\
Voxtream & 2.2 \\
WhisperSpeech & 3.9 \\
YarnGPT & 5.2 \\
ZipVoice & 3.4 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
minimax/speech-02-turbo & 6.7 \\
minimax/speech-2.6-hd & 2.1 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v11/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
speaker_similarity \\
reference_speaker \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v11/hours_per_architecture.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l r | l r | l r@{}}
\toprule
\textbf{Architecture} & \textbf{Hours} & \textbf{Architecture} & \textbf{Hours} & \textbf{Architecture} & \textbf{Hours} \\
\midrule
Azzurra-Voice & 1.5 & Llasa & 30.9 & Sesame CSM-1B & 1.7 \\
Bark & 123.3 & LongCat-AudioDiT & 3.3 & Soprano11 & 1.6 \\
Capacitron & 1.5 & LuxTTS & 1.8 & SopranoTTS & 1.7 \\
CaroTTS & 1.7 & MOSS-TTS & 41.0 & Sopro & 2.0 \\
Cartesia.ai (Sonic-3) & 3.5 & Mars5 & 1.8 & SoulX-Podcast & 1.9 \\
ChatTTS & 3.7 & MatchaTTS & 1.7 & Spark TTS & 2.1 \\
Chatterbox & 16.3 & Maya1 TTS & 2.1 & SpeechT5 & 2.0 \\
Coda & 7.3 & MegaTTS3 & 4.1 & Speedy Speech & 2.0 \\
DeepGram & 3.8 & MeloTTS & 1.8 & Step-Audio-EditX & 3.8 \\
DiT & 2.0 & Metavoice-1B & 1.9 & StyleTTS 2 & 4.1 \\
Dramabox & 3.5 & Microsoft VibeVoice & 8.3 & StyleTTS2 & 2.1 \\
Dual-AR & 19.8 & Ming-omni-tts & 3.9 & Supertonic & 17.7 \\
DualAR & 3.6 & MiniCPM-o-2.6 & 4.4 & SvaraTTS v1 & 5.2 \\
E2 TTS & 1.8 & MiniMax-Speech & 2.0 & TADA & 17.5 \\
Edge-TTS & 39.9 & MiraTTS & 2.0 & Tacotron & 2.5 \\
ElevenLabs & 10.1 & MisoTTS & 2.3 & Tacotron 2 & 20.6 \\
F5 TTS & 1.7 & NVidia Magpie-TTS & 4.5 & Tortoise & 2.1 \\
F5-TTS & 18.5 & Nari Dia-1.6B & 1.9 & VITS & 58.1 \\
FastPitch & 2.1 & Nari Dia2 & 2.1 & VITS Neon & 4.3 \\
FireRedTTS & 5.5 & NeuTTS & 2.0 & VITS-MMS & 23.3 \\
FishTTS & 7.4 & NeuTTS-Air & 2.0 & VITS2 & 1.7 \\
FreyaTTS & 1.6 & NeuralHMM & 2.1 & Veena & 3.5 \\
GLM-TTS & 2.1 & OmniVoice & 53.6 & VibeVoice & 2.0 \\
GPA & 3.5 & OpenAI TTS-1 HD & 13.7 & VieNeu-TTS & 2.3 \\
GPT-SoVITS & 2.1 & OpenVoiceV2 & 4.3 & VixTTS & 3.6 \\
Gemini & 2.5 & Openaudio-S1-Mini & 4.8 & VoXtream & 1.9 \\
GlowTTS & 12.6 & Optispeech & 1.5 & VoiceCore & 2.9 \\
Griffin Lim & 16.6 & Orpheus TTS v0.1 & 2.0 & VoxCPM & 35.6 \\
Higgs-Audio & 15.5 & OuteTTS & 15.1 & VoxCPM-1.5 & 4.1 \\
Higgs-Audio-V2 & 8.8 & Overflow & 2.2 & Voxtral & 19.1 \\
Index-TTS & 7.6 & Parler TTS & 4.9 & Voxtream & 2.2 \\
IndicF5 & 16.6 & Parler-TTS & 10.0 & WavTTS & 1.7 \\
Indri-TTS-0.1 & 3.7 & PocketTTS & 1.9 & WhisperSpeech & 3.9 \\
Inflect-Nano & 1.5 & PrimeTTS & 2.1 & XTTS v1.1 & 36.9 \\
Inworld-TTS & 3.9 & Qwen2.5-Omni & 2.3 & XTTS v2 & 38.9 \\
Jenny & 1.7 & Qwen3-Omni & 34.3 & YarnGPT & 5.2 \\
Kani-TTS & 3.8 & Qwen3-TTS & 2.3 & ZipVoice & 3.4 \\
Kitten-TTS & 4.1 & RVC & 17.6 & Zonos & 8.8 \\
Kokoro & 10.4 & Raon-OpenTTS & 1.8 & ZonosTTS v0.1 & 3.7 \\
KugelAudio & 15.6 & Resemble.ai (April 12th, 2025) & 8.8 & dots.tts & 45.5 \\
Kyutai-TTS & 4.5 & Ringg Squirrel TTS & 3.9 & minimax/speech-02 & 8.8 \\
LFM2.5-Audio & 1.8 & Sarashina & 2.2 &  &  \\
Lightning & 3.5 & Sesame CSM 1B & 2.2 &  &  \\
\bottomrule
\end{tabular*}


==> img/data_v11/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 284.3 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
openai & 13.7 \\
unknown & 718.2 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v11/hours_per_language.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l r | l r | l r@{}}
\toprule
\textbf{Language} & \textbf{Hours} & \textbf{Language} & \textbf{Hours} & \textbf{Language} & \textbf{Hours} \\
\midrule
Amharic & 3.6 & Hungarian & 12.5 & Polish & 44.5 \\
Arabic & 19.4 & Igbo & 1.8 & Portuguese & 39.2 \\
Bangla & 14.1 & Indonesian & 4.5 & Romanian & 12.8 \\
Bulgarian & 6.1 & Irish & 6.4 & Russian & 50.2 \\
Chinese & 54.6 & Italian & 57.3 & Sinhala & 2.1 \\
Croatian & 1.8 & Japanese & 29.9 & Slovak & 6.3 \\
Czech & 13.0 & Javanese & 2.4 & Slovenian & 1.8 \\
Danish & 7.7 & Kannada & 9.4 & Spanish & 66.6 \\
Dutch & 20.8 & Korean & 30.2 & Swahili & 3.4 \\
English & 286.5 & Latvian & 2.3 & Swedish & 7.4 \\
Estonian & 5.7 & Lithuanian & 2.3 & Tamil & 5.0 \\
Finnish & 13.2 & Luxembourgish & 1.7 & Thai & 7.8 \\
French & 84.6 & Malay & 2.5 & Turkish & 15.6 \\
German & 84.6 & Malayalam & 1.8 & Turkmen & 3.9 \\
Greek & 8.8 & Maltese & 8.1 & Ukrainian & 35.7 \\
Hausa & 1.5 & Marathi & 3.0 & Urdu & 2.1 \\
Hebrew & 2.0 & Norwegian & 2.0 & Vietnamese & 10.1 \\
Hindi & 22.5 & Persian & 8.8 & Yoruba & 1.8 \\
\bottomrule
\end{tabular*}


==> img/data_v11/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Audio8-TTS-Preview-0.1b & 1.8 \\
Audio8-TTS-Preview-0.6b & 1.8 \\
Ava-82M & 2.1 \\
Azzurra-Voice & 1.5 \\
CaroTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 \\
ChatTTS & 3.7 \\
Chatterbox & 1.8 \\
Chatterbox Multilingual & 10.8 \\
Chatterbox-Turbo & 1.8 \\
DeepGram & 3.8 \\
Dramabox & 3.5 \\
Echo-TTS & 2.0 \\
Edge-TTS & 39.9 \\
ElevenLabs-Turbo-v2.5 & 2.0 \\
ElevenLabs-v2-Multilingual & 4.1 \\
ElevenLabs-v3 & 4.0 \\
FireRedTTS-2.0 & 5.5 \\
Fish-S2-Pro & 19.8 \\
FishTTS & 7.4 \\
FreyaTTS & 1.6 \\
GLM-TTS & 2.1 \\
GPA-v1.0 & 1.7 \\
GPA-v1.5 & 1.8 \\
GPT-SoVITS & 2.1 \\
Gemini-3.1-Flash-TTS & 2.5 \\
Higgs-Audio-V2 & 8.8 \\
Higgs-Audio-V3 & 15.5 \\
Hume TADA-3B-ML & 14.0 \\
Index-TTS-1.5 & 4.0 \\
Index-TTS-2.0 & 3.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Inflect-Micro-v2 & 1.8 \\
Inflect-Nano-v1 & 1.5 \\
Inflect-Nano-v2 & 1.8 \\
Inworld-TTS-2 & 3.9 \\
Kani-TTS-370M & 3.8 \\
Kartoffelbox & 1.9 \\
Kitten-TTS-Nano-0.1 & 2.0 \\
Kitten-TTS-Nano-0.2 & 2.1 \\
KugelAudio & 15.6 \\
Kyutai-TTS & 4.5 \\
LEMAS-TTS & 18.5 \\
LFM2.5-Audio & 1.8 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
LongCat-AudioDiT & 3.3 \\
LuxTTS & 1.8 \\
MOSS-TTS-1.7B & 20.8 \\
MOSS-TTS-8B & 18.1 \\
MOSS-TTS-Nano-100M & 2.1 \\
Mars5 & 1.8 \\
Marvis-TTS & 1.7 \\
MatchaTTS & 1.7 \\
Maya1 TTS & 2.1 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice 1.5B & 4.1 \\
Microsoft VibeVoice Large & 4.2 \\
MingTTS & 3.9 \\
MiniCPM-o-2.6 & 4.4 \\
MiniMax-Speech-2.8-Turbo & 2.0 \\
MiraTTS & 2.0 \\
MisoTTS & 2.3 \\
NVidia Magpie-TTS Multilingual & 4.5 \\
Nari Dia-1.6B & 1.9 \\
Nari Dia2 & 2.1 \\
NeuTTS-Air & 2.0 \\
NeuTTS-Nano & 2.0 \\
OmniVoice & 53.6 \\
OpenAI TTS-1 HD & 13.7 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
OuteTTS & 15.1 \\
Parler-mini-multilingual & 10.0 \\
PocketTTS & 1.9 \\
PrimeTTS & 2.1 \\
Qwen2.5-Omni & 2.3 \\
Qwen3-TTS-12Hz-0.6B-Base & 17.3 \\
Qwen3-TTS-12Hz-1.7B-Base & 17.0 \\
Qwen3-TTS-CustomVoice & 2.3 \\
RVC & 17.6 \\
Raon-OpenTTS & 1.8 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Rime-Coda & 7.3 \\
Ringg Squirrel TTS v1.0 & 3.9 \\
Smallest-Lightning-v3.1 & 3.5 \\
Soprano11 & 1.6 \\
SopranoTTS & 1.7 \\
Sopro & 2.0 \\
SoulX-Podcast & 1.9 \\
Spark-TTS-0.5B & 2.1 \\
Step-Audio-EditX & 3.8 \\
Supertonic & 1.9 \\
SvaraTTS v1 & 5.2 \\
TADA-1B & 1.9 \\
TADA-3B-ML & 1.6 \\
Tsukasa_Speech & 4.1 \\
VITS2-Claude & 1.7 \\
Veena & 3.5 \\
VibeVoice-Realtime-0.5B & 2.0 \\
VieNeu-TTS & 2.3 \\
VoXtream2 & 1.9 \\
VoiceCore & 2.9 \\
VoxCPM-0.5B & 3.6 \\
VoxCPM-1.5 & 4.1 \\
VoxCPM2 & 32.0 \\
Voxtral & 19.1 \\
Voxtream & 2.2 \\
WavTTS & 1.7 \\
WhisperSpeech & 3.9 \\
YarnGPT & 5.2 \\
ZONOS2 & 8.8 \\
ZipVoice & 3.4 \\
dots.tts-base & 15.2 \\
dots.tts-mf & 15.1 \\
dots.tts-soar & 15.2 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
minimax/speech-02-turbo & 6.7 \\
minimax/speech-2.6-hd & 2.1 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sarashina2.2-tts & 2.2 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
supertonic-3 & 15.9 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v3/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v3/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 2.7 \\
Capacitron & 1.5 \\
FastPitch & 2.1 \\
GlowTTS & 8.1 \\
Griffin Lim & 16.6 \\
Jenny & 1.7 \\
NeuralHMM & 2.1 \\
Overflow & 2.2 \\
Parler TTS & 1.7 \\
SpeechT5 & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 2.0 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 3.9 \\
Tortoise & 2.1 \\
VITS & 39.0 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
XTTS v1.1 & 20.5 \\
XTTS v2 & 19.7 \\
\bottomrule
\end{tabular}


==> img/data_v3/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 12.2 \\
Common Voice & 17.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 19.3 \\
LibriTTS & 2.0 \\
M-AILABS & 6.2 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 65.6 \\
Sam & 2.5 \\
Thorsten & 1.8 \\
none & 16.6 \\
unknown & 4.4 \\
\bottomrule
\end{tabular}


==> img/data_v3/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 3.3 \\
Bulgarian & 2.0 \\
Czech & 2.0 \\
Danish & 1.8 \\
Dutch & 9.6 \\
English & 41.3 \\
Estonian & 1.6 \\
Finnish & 5.1 \\
French & 12.1 \\
German & 12.2 \\
Greek & 2.2 \\
Hindi & 2.4 \\
Hungarian & 6.4 \\
Irish & 2.1 \\
Italian & 12.5 \\
Maltese & 2.0 \\
Polish & 8.6 \\
Romanian & 4.5 \\
Russian & 9.6 \\
Slovak & 2.2 \\
Spanish & 7.5 \\
Swahili (macrolanguage) & 3.4 \\
Ukrainian & 9.6 \\
\bottomrule
\end{tabular}


==> img/data_v3/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
microsoft/speecht5_tts & 2.0 \\
parler_tts & 1.7 \\
suno/bark & 2.7 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 20.5 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 19.7 \\
tts_models/nl/css10/vits & 2.1 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
\bottomrule
\end{tabular}


==> img/data_v4/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v4/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 2.7 \\
Capacitron & 1.5 \\
FastPitch & 2.1 \\
GlowTTS & 8.1 \\
Griffin Lim & 16.6 \\
Jenny & 1.7 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
NeuralHMM & 2.1 \\
Overflow & 2.2 \\
Parler TTS & 1.7 \\
SpeechT5 & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 2.0 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 3.9 \\
Tortoise & 2.1 \\
VITS & 39.0 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 20.5 \\
XTTS v2 & 19.7 \\
\bottomrule
\end{tabular}


==> img/data_v4/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 12.2 \\
Common Voice & 17.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 19.3 \\
LibriTTS & 2.0 \\
M-AILABS & 6.2 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 65.6 \\
Sam & 2.5 \\
Thorsten & 1.8 \\
WhisperSpeech dataset & 3.9 \\
none & 16.6 \\
unknown & 9.9 \\
vctk & 1.7 \\
\bottomrule
\end{tabular}


==> img/data_v4/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 3.3 \\
Bulgarian & 2.0 \\
Czech & 2.0 \\
Danish & 1.8 \\
Dutch & 9.6 \\
English & 50.6 \\
Estonian & 1.6 \\
Finnish & 5.1 \\
French & 12.1 \\
German & 12.2 \\
Greek & 2.2 \\
Hindi & 2.4 \\
Hungarian & 6.4 \\
Irish & 2.1 \\
Italian & 12.5 \\
Maltese & 2.0 \\
Polish & 10.5 \\
Romanian & 4.5 \\
Russian & 9.6 \\
Slovak & 2.2 \\
Spanish & 7.5 \\
Swahili & 3.4 \\
Ukrainian & 9.6 \\
\bottomrule
\end{tabular}


==> img/data_v4/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
WhisperSpeech & 3.9 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
microsoft/speecht5_tts & 2.0 \\
parler_tts & 1.7 \\
suno/bark & 2.7 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 20.5 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 19.7 \\
tts_models/nl/css10/vits & 2.1 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
\bottomrule
\end{tabular}


==> img/data_v5/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v5/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 123.3 \\
Capacitron & 1.5 \\
E2 TTS & 1.8 \\
F5 TTS & 1.7 \\
FastPitch & 2.1 \\
GlowTTS & 12.6 \\
Griffin Lim & 16.6 \\
Jenny & 1.7 \\
Kokoro & 10.4 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
NeuralHMM & 2.1 \\
OpenVoiceV2 & 4.3 \\
Optispeech & 1.5 \\
Orpheus TTS v0.1 & 2.0 \\
Overflow & 2.2 \\
Parler TTS & 4.9 \\
Sesame CSM 1B & 2.2 \\
Spark TTS & 2.1 \\
SpeechT5 & 2.0 \\
Speedy Speech & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 4.4 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 6.9 \\
Tacotron2-DDC-GST & 3.3 \\
Tortoise & 2.1 \\
VITS & 54.4 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
VixTTS & 3.6 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 36.9 \\
XTTS v2 & 38.9 \\
ZonosTTS v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v5/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 219.2 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
unknown & 41.7 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v5/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 9.5 \\
Bangla & 9.4 \\
Bulgarian & 6.1 \\
Chinese & 14.2 \\
Croatian & 1.8 \\
Czech & 11.2 \\
Danish & 5.9 \\
Dutch & 11.5 \\
English & 83.4 \\
Estonian & 5.7 \\
Finnish & 9.2 \\
French & 19.8 \\
German & 18.8 \\
Greek & 6.7 \\
Hindi & 5.4 \\
Hungarian & 10.6 \\
Irish & 6.4 \\
Italian & 16.7 \\
Japanese & 14.5 \\
Korean & 6.2 \\
Latvian & 2.3 \\
Lithuanian & 2.3 \\
Maltese & 6.2 \\
Persian & 6.7 \\
Polish & 13.9 \\
Portuguese & 10.7 \\
Romanian & 8.7 \\
Russian & 12.6 \\
Slovak & 6.3 \\
Slovenian & 1.8 \\
Spanish & 12.5 \\
Swahili & 3.4 \\
Swedish & 5.5 \\
Thai & 3.1 \\
Turkish & 9.9 \\
Turkmen & 3.9 \\
Ukrainian & 13.7 \\
Vietnamese & 1.7 \\
\bottomrule
\end{tabular}


==> img/data_v5/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
OpenVoiceV2 & 4.3 \\
Spark-TTS-0.5B & 2.1 \\
WhisperSpeech & 3.9 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v6/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v6/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 123.3 \\
Capacitron & 1.5 \\
E2 TTS & 1.8 \\
F5 TTS & 1.7 \\
FastPitch & 2.1 \\
FishTTS & 7.4 \\
GlowTTS & 12.6 \\
Griffin Lim & 16.6 \\
Jenny & 1.7 \\
Kokoro & 10.4 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Nari Dia-1.6B & 2.1 \\
NeuralHMM & 2.1 \\
OpenVoiceV2 & 4.3 \\
Optispeech & 1.5 \\
Orpheus TTS v0.1 & 2.0 \\
Overflow & 2.2 \\
Parler TTS & 4.9 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Sesame CSM 1B & 2.2 \\
Spark TTS & 2.1 \\
SpeechT5 & 2.0 \\
Speedy Speech & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 4.4 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 6.9 \\
Tacotron2-DDC-GST & 3.3 \\
Tortoise & 2.1 \\
VITS & 54.4 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
VixTTS & 3.6 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 36.9 \\
XTTS v2 & 38.9 \\
ZonosTTS v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v6/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 219.2 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
unknown & 64.0 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v6/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 9.5 \\
Bangla & 9.4 \\
Bulgarian & 6.1 \\
Chinese & 16.0 \\
Croatian & 1.8 \\
Czech & 11.2 \\
Danish & 5.9 \\
Dutch & 11.5 \\
English & 91.9 \\
Estonian & 5.7 \\
Finnish & 9.2 \\
French & 24.3 \\
German & 23.1 \\
Greek & 6.7 \\
Hindi & 5.4 \\
Hungarian & 10.6 \\
Irish & 6.4 \\
Italian & 18.2 \\
Japanese & 14.5 \\
Korean & 6.2 \\
Latvian & 2.3 \\
Lithuanian & 2.3 \\
Maltese & 6.2 \\
Persian & 6.7 \\
Polish & 13.9 \\
Portuguese & 10.7 \\
Romanian & 8.7 \\
Russian & 12.6 \\
Slovak & 6.3 \\
Slovenian & 1.8 \\
Spanish & 14.2 \\
Swahili & 3.4 \\
Swedish & 5.5 \\
Thai & 3.1 \\
Turkish & 9.9 \\
Turkmen & 3.9 \\
Ukrainian & 13.7 \\
Vietnamese & 1.7 \\
\bottomrule
\end{tabular}


==> img/data_v6/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
FishTTS & 7.4 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Nari Dia-1.6B & 2.1 \\
OpenVoiceV2 & 4.3 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Spark-TTS-0.5B & 2.1 \\
WhisperSpeech & 3.9 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v7/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v7/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Bark & 123.3 \\
Capacitron & 1.5 \\
Chatterbox & 1.8 \\
E2 TTS & 1.8 \\
F5 TTS & 1.7 \\
FastPitch & 2.1 \\
FishTTS & 7.4 \\
GlowTTS & 12.6 \\
Griffin Lim & 16.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Jenny & 1.7 \\
Kokoro & 10.4 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Nari Dia-1.6B & 1.9 \\
NeuralHMM & 2.1 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
Optispeech & 1.5 \\
Orpheus TTS v0.1 & 2.0 \\
Overflow & 2.2 \\
Parler TTS & 4.9 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Sesame CSM 1B & 2.2 \\
Spark TTS & 2.1 \\
SpeechT5 & 2.0 \\
Speedy Speech & 2.0 \\
Tacotron DDC & 2.5 \\
Tacotron2 & 3.9 \\
Tacotron2 DCA & 4.4 \\
Tacotron2 DH & 2.0 \\
Tacotron2-DDC & 6.9 \\
Tacotron2-DDC-GST & 3.3 \\
Tortoise & 2.1 \\
VITS & 54.4 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
Veena & 3.5 \\
VixTTS & 3.6 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 36.9 \\
XTTS v2 & 38.9 \\
ZipVoice & 3.4 \\
ZonosTTS v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v7/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 235.8 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
['Multiple Datasets'] & 35.7 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
unknown & 76.3 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v7/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 9.5 \\
Bangla & 14.1 \\
Bulgarian & 6.1 \\
Chinese & 19.4 \\
Croatian & 1.8 \\
Czech & 11.2 \\
Danish & 5.9 \\
Dutch & 15.0 \\
English & 110.3 \\
Estonian & 5.7 \\
Finnish & 9.2 \\
French & 28.5 \\
German & 25.6 \\
Greek & 6.7 \\
Hindi & 12.9 \\
Hungarian & 10.6 \\
Irish & 6.4 \\
Italian & 22.0 \\
Japanese & 14.5 \\
Korean & 6.2 \\
Latvian & 2.3 \\
Lithuanian & 2.3 \\
Maltese & 6.2 \\
Marathi & 3.0 \\
Persian & 6.7 \\
Polish & 16.5 \\
Portuguese & 14.4 \\
Romanian & 8.7 \\
Russian & 12.6 \\
Slovak & 6.3 \\
Slovenian & 1.8 \\
Spanish & 16.6 \\
Swahili & 3.4 \\
Swedish & 5.5 \\
Tamil & 5.0 \\
Thai & 3.1 \\
Turkish & 9.9 \\
Turkmen & 3.9 \\
Ukrainian & 13.7 \\
Vietnamese & 1.7 \\
\bottomrule
\end{tabular}


==> img/data_v7/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Chatterbox & 1.8 \\
FishTTS & 7.4 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Nari Dia-1.6B & 1.9 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Spark-TTS-0.5B & 2.1 \\
Veena & 3.5 \\
WhisperSpeech & 3.9 \\
ZipVoice & 3.4 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v7/version.tex <==
7

==> img/data_v8/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
reference_speaker \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v8/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Azzurra-Voice & 1.5 \\
Bark & 123.3 \\
Capacitron & 1.5 \\
Chatterbox & 14.5 \\
E2 TTS & 1.8 \\
F5 TTS & 1.7 \\
FastPitch & 2.1 \\
FireRedTTS & 5.5 \\
FishTTS & 7.4 \\
GlowTTS & 12.6 \\
Griffin Lim & 16.6 \\
Higgs-Audio-V2 & 8.8 \\
Index-TTS & 7.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Jenny & 1.7 \\
Kitten-TTS & 4.1 \\
Kokoro & 10.4 \\
Kyutai-TTS & 4.5 \\
Llasa & 30.9 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice & 8.3 \\
MiniCPM-o-2.6 & 4.4 \\
NVidia Magpie-TTS & 4.5 \\
Nari Dia-1.6B & 1.9 \\
NeuralHMM & 2.1 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
Optispeech & 1.5 \\
Orpheus TTS v0.1 & 2.0 \\
OuteTTS & 15.1 \\
Overflow & 2.2 \\
Parler TTS & 4.9 \\
Qwen2.5-Omni & 2.3 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Sesame CSM 1B & 2.2 \\
Spark TTS & 2.1 \\
SpeechT5 & 2.0 \\
Speedy Speech & 2.0 \\
Tacotron & 2.5 \\
Tacotron 2 & 20.6 \\
Tortoise & 2.1 \\
VITS & 54.4 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
Veena & 3.5 \\
VixTTS & 3.6 \\
VoxCPM & 3.6 \\
Voxtream & 2.2 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 36.9 \\
XTTS v2 & 38.9 \\
ZipVoice & 3.4 \\
ZonosTTS v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v8/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 237.8 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
['Multiple Datasets'] & 46.5 \\
['unknown'] & 67.7 \\
['unknwon'] & 4.5 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
unknown & 76.3 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v8/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Arabic & 9.5 \\
Bangla & 14.1 \\
Bulgarian & 6.1 \\
Chinese & 31.2 \\
Croatian & 1.8 \\
Czech & 11.2 \\
Danish & 5.9 \\
Dutch & 15.0 \\
English & 139.8 \\
Estonian & 5.7 \\
Finnish & 9.2 \\
French & 39.5 \\
German & 35.5 \\
Greek & 6.7 \\
Hindi & 12.9 \\
Hungarian & 10.6 \\
Irish & 6.4 \\
Italian & 26.6 \\
Japanese & 14.5 \\
Korean & 11.1 \\
Latvian & 2.3 \\
Lithuanian & 2.3 \\
Maltese & 6.2 \\
Marathi & 3.0 \\
Persian & 6.7 \\
Polish & 18.3 \\
Portuguese & 14.4 \\
Romanian & 8.7 \\
Russian & 16.6 \\
Slovak & 6.3 \\
Slovenian & 1.8 \\
Spanish & 21.7 \\
Swahili & 3.4 \\
Swedish & 5.5 \\
Tamil & 5.0 \\
Thai & 3.1 \\
Turkish & 9.9 \\
Turkmen & 3.9 \\
Ukrainian & 15.9 \\
Vietnamese & 1.7 \\
\bottomrule
\end{tabular}


==> img/data_v8/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Azzurra-Voice & 1.5 \\
Chatterbox & 1.8 \\
Chatterbox Multilingual & 10.8 \\
FireRedTTS-2.0 & 5.5 \\
FishTTS & 7.4 \\
Higgs-Audio-V2 & 8.8 \\
Index-TTS-1.5 & 4.0 \\
Index-TTS-2.0 & 3.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Kartoffelbox & 1.9 \\
Kitten-TTS-Nano-0.1 & 2.0 \\
Kitten-TTS-Nano-0.2 & 2.1 \\
Kyutai-TTS & 4.5 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice 1.5B & 4.1 \\
Microsoft VibeVoice Large & 4.2 \\
MiniCPM-o-2.6 & 4.4 \\
NVidia Magpie-TTS Multilingual & 4.5 \\
Nari Dia-1.6B & 1.9 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
OuteTTS & 15.1 \\
Qwen2.5-Omni & 2.3 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Spark-TTS-0.5B & 2.1 \\
Veena & 3.5 \\
VoxCPM-0.5B & 3.6 \\
Voxtream & 2.2 \\
WhisperSpeech & 3.9 \\
ZipVoice & 3.4 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> img/data_v9/data_fields_table.tex <==
\begin{table}
\caption{Data fields per entry in the MLAAD dataset.}
\label{tab:datafields}
\begin{tabular}{|l|}
\hline
Column Names \\
\hline
index \\
path \\
original_file \\
language \\
is_original_language \\
duration \\
training_data \\
model_name \\
architecture \\
transcript \\
reference_speaker \\
len \\
\hline
\end{tabular}
\end{table}


==> img/data_v9/hours_per_architecture.tex <==
\begin{tabular}{ll}
\toprule
architecture & duration \\
\midrule
Azzurra-Voice & 1.5 \\
Bark & 123.3 \\
Capacitron & 1.5 \\
CaroTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 \\
Chatterbox & 14.5 \\
DeepGram & 3.8 \\
E2 TTS & 1.8 \\
Edge-TTS & 39.9 \\
F5 TTS & 1.7 \\
FastPitch & 2.1 \\
FireRedTTS & 5.5 \\
FishTTS & 7.4 \\
GlowTTS & 12.6 \\
Griffin Lim & 16.6 \\
Higgs-Audio-V2 & 8.8 \\
Index-TTS & 7.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Jenny & 1.7 \\
Kani-TTS & 3.8 \\
Kitten-TTS & 4.1 \\
Kokoro & 10.4 \\
Kyutai-TTS & 4.5 \\
Llasa & 30.9 \\
Mars5 & 1.8 \\
MatchaTTS & 1.7 \\
Maya1 TTS & 2.1 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice & 8.3 \\
MiniCPM-o-2.6 & 4.4 \\
NVidia Magpie-TTS & 4.5 \\
Nari Dia-1.6B & 1.9 \\
Nari Dia2 & 2.1 \\
NeuTTS-Air & 2.0 \\
NeuralHMM & 2.1 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
Optispeech & 1.5 \\
Orpheus TTS v0.1 & 2.0 \\
OuteTTS & 15.1 \\
Overflow & 2.2 \\
Parler TTS & 4.9 \\
Qwen2.5-Omni & 2.3 \\
RVC & 17.6 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Ringg Squirrel TTS & 3.9 \\
Sesame CSM 1B & 2.2 \\
Sesame CSM-1B & 1.7 \\
SoulX-Podcast & 1.9 \\
Spark TTS & 2.1 \\
SpeechT5 & 2.0 \\
Speedy Speech & 2.0 \\
Step-Audio-EditX & 3.8 \\
StyleTTS 2 & 4.1 \\
Supertonic & 1.9 \\
Tacotron & 2.5 \\
Tacotron 2 & 20.6 \\
Tortoise & 2.1 \\
VITS & 54.4 \\
VITS Neon & 4.3 \\
VITS-MMS & 23.3 \\
Veena & 3.5 \\
VieNeu-TTS & 2.3 \\
VixTTS & 3.6 \\
VoiceCore & 2.9 \\
VoxCPM & 3.6 \\
VoxCPM-1.5 & 4.1 \\
Voxtream & 2.2 \\
WhisperSpeech & 3.9 \\
XTTS v1.1 & 36.9 \\
XTTS v2 & 38.9 \\
YarnGPT & 5.2 \\
ZipVoice & 3.4 \\
ZonosTTS v0.1 & 3.7 \\
minimax/speech-02 & 8.8 \\
\bottomrule
\end{tabular}


==> img/data_v9/hours_per_dataset.tex <==
\begin{tabular}{ll}
\toprule
training_data & duration \\
\midrule
Blizzard 2013 & 1.5 \\
CSS 10 & 10.2 \\
Common Voice & 29.8 \\
EK1 & 3.9 \\
Jenny & 1.7 \\
LJSpeech & 22.8 \\
LibriTTS & 2.0 \\
M-AILABS & 7.7 \\
M-AILABS_female & 4.6 \\
M-AILABS_male & 3.7 \\
Multiple Datasets & 284.3 \\
Sam & 2.5 \\
Thorsten & 5.7 \\
VoxBox & 2.1 \\
WhisperSpeech dataset & 3.9 \\
baker & 3.3 \\
common-voice & 2.2 \\
custom & 7.9 \\
none & 16.6 \\
unknown & 265.6 \\
vctk & 1.7 \\
viVoice & 3.6 \\
\bottomrule
\end{tabular}


==> img/data_v9/hours_per_language.tex <==
\begin{tabular}{ll}
\toprule
language & duration \\
\midrule
Amharic & 3.6 \\
Arabic & 9.5 \\
Bangla & 14.1 \\
Bulgarian & 6.1 \\
Chinese & 35.2 \\
Croatian & 1.8 \\
Czech & 11.2 \\
Danish & 5.9 \\
Dutch & 15.0 \\
English & 171.3 \\
Estonian & 5.7 \\
Finnish & 9.2 \\
French & 43.6 \\
German & 44.5 \\
Greek & 6.7 \\
Hausa & 1.5 \\
Hebrew & 2.0 \\
Hindi & 15.1 \\
Hungarian & 10.6 \\
Igbo & 1.8 \\
Irish & 6.4 \\
Italian & 30.0 \\
Japanese & 21.5 \\
Javanese & 2.4 \\
Kannada & 4.2 \\
Korean & 13.7 \\
Latvian & 2.3 \\
Lithuanian & 2.3 \\
Malay & 2.5 \\
Malayalam & 1.8 \\
Maltese & 8.1 \\
Marathi & 3.0 \\
Persian & 6.7 \\
Polish & 22.4 \\
Portuguese & 14.4 \\
Romanian & 10.8 \\
Russian & 21.2 \\
Sinhala & 2.1 \\
Slovak & 6.3 \\
Slovenian & 1.8 \\
Spanish & 29.2 \\
Swahili & 3.4 \\
Swedish & 5.5 \\
Tamil & 5.0 \\
Thai & 3.1 \\
Turkish & 9.9 \\
Turkmen & 3.9 \\
Ukrainian & 20.8 \\
Urdu & 2.1 \\
Vietnamese & 4.1 \\
Yoruba & 1.8 \\
\bottomrule
\end{tabular}


==> img/data_v9/hours_per_tts_model.tex <==
\begin{tabular}{ll}
\toprule
model_name & duration \\
\midrule
Azzurra-Voice & 1.5 \\
CaroTTS & 1.7 \\
Cartesia.ai (Sonic-3) & 3.5 \\
Chatterbox & 1.8 \\
Chatterbox Multilingual & 10.8 \\
DeepGram & 3.8 \\
Edge-TTS & 39.9 \\
FireRedTTS-2.0 & 5.5 \\
FishTTS & 7.4 \\
Higgs-Audio-V2 & 8.8 \\
Index-TTS-1.5 & 4.0 \\
Index-TTS-2.0 & 3.6 \\
IndicF5 & 16.6 \\
Indri-TTS-0.1 & 3.7 \\
Kani-TTS-370M & 3.8 \\
Kartoffelbox & 1.9 \\
Kitten-TTS-Nano-0.1 & 2.0 \\
Kitten-TTS-Nano-0.2 & 2.1 \\
Kyutai-TTS & 4.5 \\
Llasa-1B & 2.3 \\
Llasa-1B-Multilingual & 24.1 \\
Llasa-3B & 2.3 \\
Llasa-8B & 2.3 \\
Mars5 & 1.8 \\
Marvis-TTS & 1.7 \\
MatchaTTS & 1.7 \\
Maya1 TTS & 2.1 \\
MegaTTS3 & 4.1 \\
MeloTTS & 1.8 \\
Metavoice-1B & 1.9 \\
Microsoft VibeVoice 1.5B & 4.1 \\
Microsoft VibeVoice Large & 4.2 \\
MiniCPM-o-2.6 & 4.4 \\
NVidia Magpie-TTS Multilingual & 4.5 \\
Nari Dia-1.6B & 1.9 \\
Nari Dia2 & 2.1 \\
NeuTTS-Air & 2.0 \\
OpenVoiceV2 & 4.3 \\
Openaudio-S1-Mini & 4.8 \\
OuteTTS & 15.1 \\
Qwen2.5-Omni & 2.3 \\
RVC & 17.6 \\
Resemble.ai (April 12th, 2025) & 8.8 \\
Ringg Squirrel TTS v1.0 & 3.9 \\
SoulX-Podcast & 1.9 \\
Spark-TTS-0.5B & 2.1 \\
Step-Audio-EditX & 3.8 \\
Supertonic & 1.9 \\
Tsukasa_Speech & 4.1 \\
Veena & 3.5 \\
VieNeu-TTS & 2.3 \\
VoiceCore & 2.9 \\
VoxCPM-0.5B & 3.6 \\
VoxCPM-1.5 & 4.1 \\
Voxtream & 2.2 \\
WhisperSpeech & 3.9 \\
YarnGPT & 5.2 \\
ZipVoice & 3.4 \\
e2-tts & 1.8 \\
f5-tts & 1.7 \\
facebook/mms-tts-deu & 1.9 \\
facebook/mms-tts-eng & 2.0 \\
facebook/mms-tts-fin & 2.6 \\
facebook/mms-tts-fra & 1.9 \\
facebook/mms-tts-hun & 2.0 \\
facebook/mms-tts-nld & 2.5 \\
facebook/mms-tts-ron & 2.5 \\
facebook/mms-tts-rus & 2.1 \\
facebook/mms-tts-swe & 3.4 \\
facebook/mms-tts-ukr & 2.4 \\
griffin_lim & 16.6 \\
kokoro & 10.4 \\
microsoft/speecht5_tts & 2.0 \\
minimax/speech-02-turbo & 6.7 \\
minimax/speech-2.6-hd & 2.1 \\
optispeech & 1.5 \\
orpheus-tts-0.1-finetune & 2.0 \\
parler_tts_large_v1 & 1.6 \\
parler_tts_mini_v0.1 & 1.7 \\
parler_tts_mini_v1 & 1.6 \\
sesame_csm & 2.2 \\
suno/bark & 2.6 \\
suno/bark-small & 2.6 \\
tts_models/bg/cv/vits & 2.0 \\
tts_models/bn/custom/vits-female & 2.6 \\
tts_models/bn/custom/vits-male & 3.0 \\
tts_models/cs/cv/vits & 2.0 \\
tts_models/da/cv/vits & 1.8 \\
tts_models/de/css10/vits-neon & 2.2 \\
tts_models/de/thorsten/tacotron2-DCA & 2.4 \\
tts_models/de/thorsten/tacotron2-DDC & 1.6 \\
tts_models/de/thorsten/vits & 1.8 \\
tts_models/el/cv/vits & 2.2 \\
tts_models/en/blizzard2013/capacitron-t2-c50 & 1.5 \\
tts_models/en/ek1/tacotron2 & 3.9 \\
tts_models/en/jenny/jenny & 1.7 \\
tts_models/en/ljspeech/fast_pitch & 2.1 \\
tts_models/en/ljspeech/glow-tts & 2.2 \\
tts_models/en/ljspeech/neural_hmm & 2.1 \\
tts_models/en/ljspeech/overflow & 2.2 \\
tts_models/en/ljspeech/speedy-speech & 2.0 \\
tts_models/en/ljspeech/tacotron2-DCA & 2.0 \\
tts_models/en/ljspeech/tacotron2-DDC & 2.4 \\
tts_models/en/ljspeech/tacotron2-DDC_ph & 2.0 \\
tts_models/en/ljspeech/vits & 2.2 \\
tts_models/en/ljspeech/vits--neon & 2.1 \\
tts_models/en/multi-dataset/tortoise-v2 & 2.1 \\
tts_models/en/sam/tacotron-DDC & 2.5 \\
tts_models/es/css10/vits & 1.7 \\
tts_models/es/mai/tacotron2-DDC & 1.4 \\
tts_models/et/cv/vits & 1.6 \\
tts_models/fa/custom/glow-tts & 2.3 \\
tts_models/fi/css10/vits & 2.5 \\
tts_models/fr/css10/vits & 1.8 \\
tts_models/fr/mai/tacotron2-DDC & 1.5 \\
tts_models/ga/cv/vits & 2.1 \\
tts_models/hr/cv/vits & 1.8 \\
tts_models/hu/css10/vits & 2.0 \\
tts_models/it/mai_female/glow-tts & 1.5 \\
tts_models/it/mai_female/vits & 1.6 \\
tts_models/it/mai_male/glow-tts & 1.6 \\
tts_models/it/mai_male/vits & 2.1 \\
tts_models/lt/cv/vits & 2.3 \\
tts_models/lv/cv/vits & 2.3 \\
tts_models/mt/cv/vits & 2.0 \\
tts_models/multilingual/multi-dataset/bark & 118.0 \\
tts_models/multilingual/multi-dataset/xtts_v1.1 & 36.9 \\
tts_models/multilingual/multi-dataset/xtts_v2 & 38.9 \\
tts_models/pl/mai_female/vits & 1.6 \\
tts_models/pt/cv/vits & 2.1 \\
tts_models/ro/cv/vits & 1.9 \\
tts_models/sk/cv/vits & 2.2 \\
tts_models/sl/cv/vits & 1.8 \\
tts_models/sv/cv/vits & 1.6 \\
tts_models/tr/common-voice/glow-tts & 2.2 \\
tts_models/uk/mai/glow-tts & 2.8 \\
tts_models/uk/mai/vits & 1.9 \\
tts_models/zh-CN/baker/tacotron2-DDC-GST & 3.3 \\
vixTTS & 3.6 \\
zonosTTS-v0.1 & 3.7 \\
\bottomrule
\end{tabular}


==> tables/v1/quality.tex <==
\begin{tabular}{lrr}
\toprule
label &   original &         fake \\
\midrule
Arabic        &            &    2.3 ± 4.9 \\
Bulgarian     &            &   8.1 ± 26.5 \\
Czech         &            &    4.2 ± 4.4 \\
Danish        &            &   10.7 ± 7.2 \\
German        &            &    1.6 ± 4.7 \\
Greek         &            &    6.5 ± 9.1 \\
English       &  0.5 ± 1.9 &   3.2 ± 10.7 \\
Spanish       &            &    0.9 ± 2.4 \\
Estonian      &            &    4.3 ± 3.8 \\
Finnish       &            &    0.8 ± 1.4 \\
French        &            &    2.3 ± 6.1 \\
Hindi         &            &    7.3 ± 7.6 \\
Hungarian     &            &    2.7 ± 3.5 \\
Italian       &            &    4.8 ± 5.8 \\
Maltese       &            &  16.8 ± 11.1 \\
Dutch         &            &  11.4 ± 23.0 \\
Romanian      &            &    2.5 ± 3.2 \\
Russian       &            &    2.3 ± 4.1 \\
Slovak        &            &    4.4 ± 3.9 \\
Swedish       &            &    6.3 ± 6.2 \\
Ukrainian     &            &  16.0 ± 17.8 \\
\textbf{Mean} &  0.5 ± 1.9 &   4.5 ± 10.9 \\
\bottomrule
\end{tabular}

==> tables/v1/tab1.tex <==
\begin{tabular}{llllllllll}
\toprule
Model &             Train Data & ASVspoof19 & ASVspoof21-DF & ASVspoof21-LA & FakeOrReal & InTheWild & MLAD & Voc.v & WaveFake \\
\midrule
  SSL-W2V2 &    ASV19 &                           - &                    \cellcolor{blue!15}         96.0±1.0 &                             - &               \cellcolor{blue!15}         91.6±1.7 &               \cellcolor{blue!15}         89.2±0.2 &              \cellcolor{blue!15}            83.0±1.3 &                          64.2±7.2 &                            21.7±10.5 \\
  &      FOR &                          50.2±3.5 &                             74.4±3.1 &                             70.7±1.9 &                         - &                        53.4±2.9 &                          65.2±8.4 &                           3.2±2.9 &                              0.0±0.0 \\
   &      ITW &                         78.1±12.5 &                            74.8±10.9 &                             68.8±9.4 &                       68.5±14.8 &                         - &                          60.4±8.0 &                         44.0±27.1 &                            69.9±34.4 \\
   &    MLAAD &                         71.0±17.0 &                             73.2±4.1 &                         \cellcolor{blue!15}    76.1±4.7 &                        51.5±1.0 &                        51.3±3.0 &                           - &                         70.2±14.6 &  \cellcolor{blue!15}    100.0±0.0 \\
  \midrule
 WhisperDF &    ASV19 &                           - &                             81.2±1.4 &                             - &                        78.3±2.9 &                        70.7±7.6 &                          79.2±4.5 &                          25.0±5.8 &                            10.2±17.0 \\
 &      FOR &                         53.1±21.0 &                             63.4±7.4 &                             61.8±7.2 &                         - &                        57.0±8.4 &                          56.9±7.4 &                          9.9±14.6 &                              2.6±4.3 \\
 &      ITW &                          65.0±3.8 &                             64.0±4.0 &                             59.1±5.0 &                        61.1±1.7 &                         - &                          55.6±3.2 &                         46.2±15.0 &                            43.2±23.7 \\
 &    MLAAD &             \cellcolor{blue!15}             80.1±2.2 &                             57.3±3.2 &                             63.3±5.1 &                        57.1±2.9 &                        62.4±6.0 &                           - &                         61.0±17.4 &                             94.5±3.8 \\
 \midrule
RawGat-ST & ASV19 &                           - &                            59.8±15.4 &                            - &                       60.6±14.2 &                        53.8±3.4 &                         55.2±13.3 &                         23.8±21.6 &                            33.5±29.3 \\
&   FOR &                          46.2±9.5 &                             56.9±4.9 &                             63.0±7.3 &                         - &                        49.8±0.3 &                          51.2±1.0 &                           2.3±2.2 &                              0.0±0.0 \\
 &   ITW &                         59.3±12.0 &                             53.8±7.0 &                             52.9±5.6 &                        57.0±7.9 &                         - &                         55.1±13.5 &                         65.1±27.3 &                            70.0±23.3 \\
 & MLAAD &                          67.4±3.2 &                             61.8±2.6 &                             59.2±2.2 &                        68.6±3.4 &                        65.8±4.8 &                           - &                         \cellcolor{blue!15} 74.9±18.3 &                            58.3±21.8 \\

\bottomrule
\end{tabular}

==> tables/v2/ed_and_mos.tex <==
\begin{tabular}{l|rr|rr}
\toprule
label &      fake_ed & original_ed &   fake_mos & original_mos \\
\midrule
Arabic        &    8.0 ± 5.4 &             &  4.2 ± 0.1 &              \\
Bulgarian     &  14.4 ± 34.4 &             &  4.1 ± 0.1 &              \\
Czech         &    6.6 ± 4.9 &             &  4.1 ± 0.1 &              \\
Danish        &  25.9 ± 13.1 &             &  4.1 ± 0.0 &              \\
German        &    2.6 ± 2.9 &   3.3 ± 6.9 &  4.0 ± 0.4 &    3.8 ± 0.5 \\
Greek         &  16.6 ± 27.3 &             &  4.2 ± 0.1 &              \\
English       &    5.3 ± 5.9 &   3.0 ± 4.1 &  4.0 ± 0.3 &    4.1 ± 0.1 \\
Spanish       &    2.4 ± 3.0 &   2.1 ± 2.5 &  4.1 ± 0.2 &    4.0 ± 0.2 \\
Estonian      &    7.7 ± 5.7 &             &  4.1 ± 0.1 &              \\
Finnish       &    2.5 ± 2.1 &             &  4.0 ± 0.1 &              \\
French        &    5.5 ± 7.7 &   3.7 ± 4.0 &  4.1 ± 0.2 &    4.0 ± 0.2 \\
Hindi         &  17.1 ± 32.2 &             &  4.1 ± 0.2 &              \\
Hungarian     &    5.7 ± 4.4 &             &  4.1 ± 0.1 &              \\
Italian       &   9.5 ± 10.0 &   2.1 ± 2.3 &  4.1 ± 0.1 &    4.0 ± 0.1 \\
Maltese       &  42.1 ± 17.3 &             &  4.1 ± 0.1 &              \\
Dutch         &    6.0 ± 5.1 &             &  4.1 ± 0.1 &              \\
Polish        &   5.5 ± 13.5 &   2.6 ± 3.0 &  4.0 ± 0.3 &    4.0 ± 0.2 \\
Romanian      &    7.5 ± 5.9 &             &  4.1 ± 0.1 &              \\
Russian       &    5.6 ± 5.7 &   3.1 ± 3.5 &  4.1 ± 0.1 &    4.1 ± 0.1 \\
Slovak        &    9.6 ± 6.1 &             &  4.1 ± 0.1 &              \\
Swahili            &  32.5 ± 16.1 &             &  4.2 ± 0.0 &              \\
Ukrainian     &  21.9 ± 33.3 &  5.7 ± 10.9 &  4.1 ± 0.2 &    4.1 ± 0.1 \\
\textbf{Mean} &    11.8±18.1 &     3.1±5.1 &    4.1±0.2 &      4.0±0.3 \\
\bottomrule
\end{tabular}

==> tables/v2/quality.tex <==
\begin{tabular}{lrr}
\toprule
 &         Fake &    Original \\
\midrule
Arabic        &    8.0 ± 5.3 &             \\
Bulgarian     &  15.1 ± 37.8 &             \\
Czech         &    5.8 ± 4.3 &             \\
Danish        &  25.8 ± 13.7 &             \\
Dutch         &    6.9 ± 5.3 &             \\
German        &    2.4 ± 2.6 &   3.5 ± 7.4 \\
Greek         &  16.0 ± 27.2 &             \\
English       &    4.5 ± 4.9 &   2.8 ± 3.7 \\
Estonian      &    7.8 ± 6.1 &             \\
Finnish       &    2.3 ± 2.0 &             \\
French        &    4.8 ± 5.1 &   4.0 ± 4.3 \\
Hindi         &  18.7 ± 34.7 &             \\
Hungarian     &    5.9 ± 4.3 &             \\
Italian       &   9.5 ± 10.4 &   2.0 ± 2.0 \\
Maltese       &  41.8 ± 17.4 &             \\
Polish        &   5.8 ± 14.0 &   2.7 ± 3.1 \\
Romanian      &    6.9 ± 5.4 &             \\
Russian       &    4.9 ± 4.6 &   2.9 ± 3.6 \\
Slovak        &    9.3 ± 5.9 &             \\
Spanish       &    2.5 ± 3.1 &   2.1 ± 2.5 \\
Swahili            &  33.2 ± 16.8 &             \\
Ukrainian     &  23.2 ± 34.0 &  6.1 ± 11.3 \\
\textbf{Mean} &  11.9 ± 18.9 &   3.1 ± 5.3 \\
\bottomrule
\end{tabular}
